ScaleBiO: Scalable Bilevel Optimization for LLM Data Reweighting

Bilevel optimization has shown its utility across various machine learning settings, yet most algorithms in practice require second-order information, making it challenging to scale them up. Only recently, a paradigm of first-order algorithms has emerged in the theoretical literature, capable of effectively addressing bilevel optimization problems. Nevertheless, the practical efficiency of this paradigm remains unverified, particularly in the context of large language models (LLMs). This paper introduces the first scalable instantiation of this paradigm called ScaleBiO, focusing on bilevel optimization for large-scale LLM data reweighting. By combining with a recently proposed memory-efficient training technique called LISA, our novel algorithm allows the paradigm to scale to $\sim$30B-sized LLMs on $8\times$H100 GPUs, marking the first successful application of bilevel optimization under practical scenarios for large-sized LLMs. Empirically, extensive experiments on data reweighting verify the effectiveness of ScaleBiO for different-scaled models, including Llama-3-8B, Gemma-2-9B, Qwen-2-7B, and Qwen-2.5-32B, where bilevel optimization succeeds in instruction-following and math reasoning tasks, outperforming several popular baselines, including uniform sampling, influence-aware data filtering, and reference-model-based sampling methods. Theoretically, ScaleBiO ensures the optimality of the learned data weights, along with a convergence guarantee matching the conventional first-order bilevel optimization paradigm on smooth and strongly convex objectives.

==> Deprecated/deprecated.tex <==
\subsubsection{Large-Scale Data Reweighting}

\input{tables/tb_weight}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Image/exp_yi.pdf}
    \caption{Learned weights in large-scale data reweighting experiments for Yi-34B. We focus on the top 5 data sources and denote the remaining as Others.}
    \label{fig:weight-34b}
\end{figure}

To demonstrate ScaleBiO's effectiveness in large-scale settings, practical choices of model and datasets are employed under the data reweighting scenarios. Specifically, we collect popular instruction following and chat completion data to construct a diverse training dataset of 18 distinct sources. The training set is formed by 9 high-quality datasets that are mostly from GPT-4 and 9 multilingual datasets serving as less relevant data sources. For our reference dataset $\mD_\text{val}$, we prompt GPT-4 to generate 1200 two-turn instructions and responses that correspond to the 8 categories in MT-Bench. Our detailed data description and preprocessing can be found in Appendix \ref{sec:appendix:large_scale_exp_setup}.

We test our approach on LLaMA-3 model series\footnote{\url{https://ai.meta.com/blog/meta-llama-3/}} with parameter size of 8B and 13B\footnote{\url{https://huggingface.co/Replete-AI/Llama-3-13B}}. We also conduct experiments on GPT-NeoX-20B~\citep{gpt-neox-20b} and Yi-34B~\citep{ai2024yi}. To evaluate our approach, we first sample 3,000 data from each source for reweighting. Then we sample 10,000 data according to the weights at the end of bilevel optimization to train our model (denotes as \textit{Ours}). For a fair baseline comparison, we sample 10,000 data uniformly and add the reference data $\mD_\text{val}$ into them to train the baseline model (denotes as \textit{Baseline}).

As shown in Table~\ref{tab:tb-weight} and Figure~\ref{fig:weight-34b}, for models with sizes varied from 8B to 34B, ScaleBiO is capable of filtering out the most irrelevant multi-lingual datasets and putting emphasis on GPT-4 generated data sources. Strikingly, the top three weights in all models were found to be within a small subset of our numerous data sources (WildChat, Airoboros, ChatAlpaca and ShareGPT4), which suggests a universality in the importance attributed to these data sources. Moreover, the top three weights in all models account for over 80\% of the total weight. This concentration of importance in a small subset of data sources highlights the effectiveness of our method in identifying and emphasizing the most influential data sources, indicating that our method consistently identifies the most critical data sources, regardless of the model architecture.

\subsubsection{Large Scale Instruction Following}

To confirm the gain of ScaleBiO, we further apply learned sampling weights to fine-tune LLaMA-3-8B and LLaMA-3-70B models.

We evaluate LLMs' instruction-following ability using MT-Bench~\cite{zheng2023judging} with single-answer grading. This benchmark prompts chat assistants with challenging multi-turn open-ended questions and uses "LLM-as-a-judge" for evaluation. MT-Bench stands out as a comprehensive benchmark that aligns well with human preference. It comprises 80 questions, evenly distributed across 8 categories: Writing, Roleplay, Extraction, Reasoning, Math, Coding, Knowledge I (STEM), and Knowledge II (humanities/social science). To demonstrate, we compare the performance of LLaMA-3-8B trained with our reweighted data versus the original data. Specifically, we first reweight data sources on LLaMA-3-8B. Then we fune-tune the LLM using the reweighted data.

The results, as shown in Table~\ref{tab:70B} and Table~\ref{tab:main}, indicate that our method consistently outperforms the baseline across different categories by a large margin, highlighting the effectiveness of our reweighting approach.

On top of that, the same weights learned from LLaMA-3-8B can be seamlessly transferred to fine-tuning LLaMA-3-70B model. As shown in Table~\ref{tab:70B}, our model achieves noticeable improvement on average compared with the baseline, proving the transferability of the learned data weights across the same family of models.

\input{tables/tb_70B}

\subsubsection{Implementation Details} Our data reweighting process lasts for 3 epochs with $\alpha$ equals to 100 and initial learning rate of $10^{-5}$ for models and $10^{-2}$ for weights. For all our fine-tuning processes, we train the LLM for 1 epoch with an initial learning rate of $8\times 10^{-6}$ and a global batch size of 64. Throughout our experiments, we adopt randomized coordinate descent with AdamW~\citep{pan2024lisa} and bfloat16 precision for efficient training and inference. Our experiments are conducted on 8 NVIDIA A100 80GB GPUs.

% \paragraph{Our method produces transferable data weights across models.} 
% To see how our weights transfers, we reweight data sources on LLaMA-3-8B as in the previous experiment, then we 

% \paragraph{Less than 20\% data sources accounts for over 80\% importance.} 
% We assess the similarity and consistency of the data weights for models in different series and different size. Specifically, we compare data reweighting results on LLaMA-3-8B, LLaMA-3-13B\footnote{\url{https://huggingface.co/Replete-AI/Llama-3-13B}}, GPT-NeoX-20B and Yi-34B. We present the top 3 data sources with the largest weights in Table~\ref{tab:tb-weight}. Strikingly, the top three weights in all models were found to be within a small subset of our numerous data sources (WildChat, Airoboros, ChatAlpaca and ShareGPT4), suggests a universality in the importance attributed to these data sources. Moreover, the top three weights in all models account for over 80\% of the total weight. This concentration of importance in a small subset of data sources highlights the effectiveness of our method in identifying and emphasizing the most influential data sources, indicating that our method consistently identifies the most critical data sources, regardless of the model architecture.

% \paragraph{Our method is highly scalable, supporting data reweighting over 30 billion parameter models.} To validate the scalability of our method, we reweight data sources on Yi-34Bs. We plot the weights as functions of step during bilevel optimization in Figure~\ref{fig:weight-34b}. We observe that the learning curve for the weights is smooth and converge at the end of training. At the same time, as shown in Table~\ref{tab:tb-weight}, ScaleBiO is capable of selecting informative data samples for the task and model, while filtering irrelevant samples.

% \section{Discussion}

\subsection{Detailed MT-Bench Scores for LLaMA}

The detailed MT-Bench scores for LLaMA-3-8B in Section~\ref{sec:appendix:large_scale_exp_setup} are provided in Table~\ref{tab:main}.
\input{tables/tb_scale_model}


\subsection{Data Hyper-Cleaning on MNIST}
% \subsection{Data Hyper-Cleaning on MNIST}\label{sec:num:hyper:clean}

We also provide additional experiments on MNIST to compare ScaleBiO with conventional bilevel optimization algorithms. Here data hyper-cleaning aims at cleaning the dataset with corrupted labels via reweighting
\begin{align*}
   \min_{\lambda} \quad  & \quad L_1(\lambda; S_{\text{val}}) = \sum_{j\in S_{\text{val}}}\ell(u_{\ast}(\lambda);\xi_j)\notag \\
  s.t., \quad  & \quad  u^{\ast}(\lambda) = \arg\min_{u} L_2(\lambda, u; S_{\text{str}}) =  \sum_{i \in S_{\text{str}}} \sigma(\lambda_i) \ell(u; \xi_{i}) + c \left\|u \right\|^2
\end{align*}
where $\sigma(\lambda_i):= \text{sigmoid}(\lambda_i)$, $\ell(x)$ is the loss function, $\lambda \in \R^m$ with $m = |S_{\text{str}}|$ and $c>0$ being a constant. We consider a subset of MNIST with 20000 examples for training, 5000 examples for validation, and 10000 examples for testing. The setting is similar to Section 6 of~\citet{ji2021bilevel} except for the model choice, where we use a non-linear model of two-layer neural networks with 0.2 dropouts instead of logistic regression. For the baseline, we compare three bilevel methods: (1) stocBiO~\citep{ji2021bilevel}, which is the stochastic bilevel method and uses Neumann series approximation to obtain sample-efficient hyper-gradient estimator; (2) truncated reverse method; (3) conjugate gradient (CG) method. The weight-decay parameter is fixed to be $c=0.001$. We sample both inner and outer problems by mini-batch for stocBiO and the full coordinates update of Algorithm~\ref{alg:minmax:sgd}. For reverse and CG methods, we employ gradient descent to optimize the inner and outer problems, as their stochastic counterparts are not easily accessible. The test accuracy of each method under different noise levels $p$ is presented in Figure~\ref{fig:hyper:noise} and the time of each algorithm to reach 90\% test accuracy is recorded in Table~\ref{tab:time:noise}. All those results demonstrate that our method is capable of reaching a relatively high accuracy with a much shorter time than others.

 \begin{figure}[h]
     \centering 
\includegraphics[width=0.3\textwidth,height=1.6in]{Image/hyper_data_cleaning_noise_01.pdf}
\includegraphics[width=0.3\textwidth,height=1.6in]{Image/hyper_data_cleaning_noise_03.pdf}
\includegraphics[width=0.3\textwidth,height=1.6in]{Image/hyper_data_cleaning_noise_05.pdf}
 \caption{Data cleaning results on MNIST}
\label{fig:hyper:noise}
\end{figure}


\begin{table}[h]
  \centering
   %  \parbox{.45\linewidth}{
    \small
    \begin{tabular}{c|rrrr}
     \toprule
        \multirow{2}{*}{Noise} &  \multicolumn{4}{c}{Time (s)} \\   
          &  ScaleBiO & stocBiO  & Reverse & CG\\ \midrule
  $p = 0.1$   & \textbf{48} & 95 & 3163 & 3428\\ \midrule 
      $p=0.3$  & \textbf{96} & --    & 4675      &  4113\\\midrule  
      $p=0.5$  &  \textbf{137} & -- & 7947 & 6084 \\ \bottomrule 
     \end{tabular}
     \caption{Time of test accuracy reaching 90\%, ``-'' means the method fails to reach this accuracy} 
     \label{tab:time:noise}
\end{table}

==> tables/tb_scale_model.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]\small
	\renewcommand    
	\arraystretch{1.3}
	\centering
        \resizebox{\linewidth}{!}{
            \setlength{\tabcolsep}{1.5mm}
\begin{tabular}{l l c c c c c c c c c}
\toprule
\multicolumn{2}{c}{Model}              & Coding & Extraction & Humanities            & Math & Reasoning & Roleplay & STEM  & Writing & Average  \\ \midrule
\multirow{2}{*}{Llama-3-8B}  & \textit{Baseline}     & 4.65   & 6.20        & 7.50                   & 3.40  & 5.25      & 7.70      & 7.00   & 7.20     & 6.11  \\
                        &  \textit{Ours}  & \textbf{5.40}    & \textbf{8.55}       & \textbf{9.68}                 & \textbf{3.45} & \textbf{5.30}       & \textbf{8.20}      & \textbf{8.73} & \textbf{7.63}   & \textbf{7.12}  \\
% \multirow{2}{*}{LLaMA-3-70B} & \textit{Baseline}  & 5.75  &  7.43  &  9.90 & 5.45  & 7.30 & 8.55 & 9.00 & 9.55 & 7.85  \\
%                             & \textit{Ours}     &  \textbf{6.40} & \textbf{8.45} & 9.85  & \textbf{6.60} &  6.60 & 8.10 & \textbf{9.50} & 8.90  &  \textbf{8.05}  \\
\bottomrule
\end{tabular}
}
\caption{Comparison of our approach and the baseline on MT-Bench.}
\label{tab:main}
\end{table*}
